Live Laparoscopic Video Retrieval with Compressed Uncertainty

Searching through large volumes of medical data to retrieve relevant information is a challenging yet crucial task for clinical care. However the primitive and most common approach to retrieval, involving text in the form of keywords, is severely limited when dealing with complex media formats. Content-based retrieval offers a way to overcome this limitation, by using rich media as the query itself. Surgical video-to-video retrieval in particular is a new and largely unexplored research problem with high clinical value, especially in the real-time case: using real-time video hashing, search can be achieved directly inside of the operating room. Indeed, the process of hashing converts large data entries into compact binary arrays or hashes, enabling large-scale search operations at a very fast rate. However, due to fluctuations over the course of a video, not all bits in a given hash are equally reliable. In this work, we propose a method capable of mitigating this uncertainty while maintaining a light computational footprint. We present superior retrieval results (3-4 % top 10 mean average precision) on a multi-task evaluation protocol for surgery, using cholecystectomy phases, bypass phases, and coming from an entirely new dataset introduced here, critical events across six different surgery types. Success on this multi-task benchmark shows the generalizability of our approach for surgical video retrieval.

==> tables/ec_split.tex <==
\begin{table}
  \centering
  \begin{tabular}{r || c|c|c}
          &  Bypass40  & Cholec80 & CEV64  \\ \hline
Query     & 284  & 307 & 580 \\
Codebook  & 1409 & 928 & 1659 \\\hline
Training  & \multicolumn{3}{c}{\textbf{81000}} \\
Validation& \multicolumn{3}{c}{\textbf{16000}} \\
\end{tabular}
\caption{Data splitting for all three test protocols. Note that the training set and validation set are common to all three.}
\label{tab:ec_split}
\end{table}

